Safe Reach Set Computation via Neural Barrier Certificates

We present a novel technique for online safety verification of autonomous systems, which performs reachability analysis efficiently for both bounded and unbounded horizons by employing neural barrier certificates. Our approach uses barrier certificates given by parameterized neural networks that depend on a given initial set, unsafe sets, and time horizon. Such networks are trained efficiently offline using system simulations sampled from regions of the state space. We then employ a meta-neural network to generalize the barrier certificates to state space regions that are outside the training set. These certificates are generated and validated online as sound over-approximations of the reachable states, thus either ensuring system safety or activating appropriate alternative actions in unsafe scenarios. We demonstrate our technique on case studies from linear models to nonlinear control-dependent models for online autonomous driving scenarios.

==> figures/cegis-structure.tex <==
\begin{figure}
\centering
\begin{tikzpicture}
%\draw [help lines] (0,0) grid (9,9);
\node (learner) [draw, rectangle, rounded corners, minimum width=1.5cm, minimum height =0.75cm]
	at (0,2) {Learner};

\node (verif) [draw, rectangle, rounded corners, minimum width=1.5cm, minimum height =0.75cm]
	at (3,2) {Verifier};

\node (out) [] at (5,2) {} ;


\draw [->, bend left] (verif) edge node[below] {\texttt{counter-example}} (learner);

\draw [->, bend left] (learner) edge node[above] {\normalsize Candidate} (verif);

\draw[->] (verif) edge node[above] {\texttt{valid}} (out);

\end{tikzpicture}
  \caption{The Counter-Example Guided Inductive Synthesis (CEGIS) loop. }
  \label{fig:basic-cegis}
\end{figure}


==> figures/ff-nn.tex <==
\begin{figure}
  \centering
  \begin{tikzpicture}%[inner sep=2pt, minimum size=0.5cm]
    % [%
    % relu/.pic={
    %   \draw (0,0) -- (0.25,0)
    %   (0.25,0) -- (0.5,0.25);}
    % ]
    %\draw [help lines] (0,0) grid (9,9);

    % input layer
    \node (x1) [ draw, circle, inner sep=2pt, minimum size=0.5cm]
    at (0,1) {};
    \node (x2) [ draw, circle, inner sep=2pt, minimum size=0.5cm]
    at (0,0) {};
    
    % input vector
    \node (x1-name) [] at (-0.5,1) {$x_1$};
    \node (x2-name) [] at (-0.5,0) {$x_2$};
    
    % hidden layer
    \node (z1) [ draw, circle, inner sep=2pt, minimum size=0.5cm]
    at (2,1.5) {$\sigma_1$};
    \node (z2) [ draw, circle, inner sep=2pt, minimum size=0.5cm]
    at (2,0.5) {$\sigma_1$};
    \node (z3) [draw, circle, inner sep=2pt, minimum size=0.5cm] at (2, -0.5){$\sigma_1$} ;

    % output layter
    \node (y) [ draw, circle, minimum size=0.5cm]
    at (4,0.5) {};
    
    % outut
    \node (y-name) [] at (4.75,0.5) {$\mathcal{N}(x)$};
    

    % \node (b1) [inner sep=0pt] at (1.75,2) {$b_1$};
    % \node (b2) [inner sep=0pt] at (1.75,-.5) {$b_2$};
    
    % connections
    \draw [->] (x1) edge node[above] {} (z1);
    \draw [->] (x1) edge node[below, pos=0.7] {} (z2);
    \draw [->] (x1) edge node[below, pos=0.7] {} (z3);
    
    \draw [->] (x2) edge node[above, pos=0.7] {} (z1);
    \draw [->] (x2) edge node[below] {} (z2);
    \draw [->] (x2) edge node[below] {} (z3);

    \draw [->] (z1) edge node[above] {} (y);
    \draw [->] (z2) edge node[below] {} (y);
    \draw [->] (z3) edge node[below] {} (y);
    

	
    
  \end{tikzpicture}
  \caption{A feed-forward neural network with two input neurons, one hidden layer and a single output neuron.}
  \label{fig:ff-nn}
\end{figure}

==> figures/scheme.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-0.8,xscale=0.9]
%uncomment if require: \path (0,310); %set diagram left start at 0, and has height of 310

%Rounded Rect [id:dp9043407638554077] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.39 ] (100,110) .. controls (100,105.58) and (103.58,102) .. (108,102) -- (162,102) .. controls (166.42,102) and (170,105.58) .. (170,110) -- (170,134) .. controls (170,138.42) and (166.42,142) .. (162,142) -- (108,142) .. controls (103.58,142) and (100,138.42) .. (100,134) -- cycle ;
%Rounded Rect [id:dp7185147457687526] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.39 ] (238.42,89.6) .. controls (238.42,80.98) and (245.41,74) .. (254.02,74) -- (326.9,74) .. controls (335.52,74) and (342.5,80.98) .. (342.5,89.6) -- (342.5,136.4) .. controls (342.5,145.02) and (335.52,152) .. (326.9,152) -- (254.02,152) .. controls (245.41,152) and (238.42,145.02) .. (238.42,136.4) -- cycle ;
%Straight Lines [id:da2020278639801083] 
\draw    (172.5,122) -- (230.88,122) ;
\draw [shift={(232.88,122)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da6217734712150864] 
\draw    (46.5,123) -- (93.5,123) ;
\draw [shift={(95.5,123)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da16928491891693276] 
\draw    (69.5,94) -- (69,123) ;
%Straight Lines [id:da7472083410962254] 
\draw    (69.5,94) -- (229.5,93.01) ;
\draw [shift={(231.5,93)}, rotate = 539.65] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da14777191788690702] 
\draw    (374.5,117) -- (374.5,164) ;
\draw [shift={(374.5,166)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp0017286098717381737] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=0.58 ] (304,186.6) .. controls (304,179.09) and (310.09,173) .. (317.6,173) -- (400.9,173) .. controls (408.41,173) and (414.5,179.09) .. (414.5,186.6) -- (414.5,227.4) .. controls (414.5,234.91) and (408.41,241) .. (400.9,241) -- (317.6,241) .. controls (310.09,241) and (304,234.91) .. (304,227.4) -- cycle ;
%Straight Lines [id:da5335793150286228] 
\draw    (263.5,206) -- (293.5,206) ;
\draw [shift={(295.5,206)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da08818983024873694] 
\draw    (348,117) -- (374.5,117) ;
%Straight Lines [id:da6594129080309898] 
\draw    (421,208) -- (480.5,208) ;
\draw [shift={(482.5,208)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp7670233648259084] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (489,182.8) .. controls (489,174.63) and (495.63,168) .. (503.8,168) -- (563.7,168) .. controls (571.87,168) and (578.5,174.63) .. (578.5,182.8) -- (578.5,227.2) .. controls (578.5,235.37) and (571.87,242) .. (563.7,242) -- (503.8,242) .. controls (495.63,242) and (489,235.37) .. (489,227.2) -- cycle ;
%Straight Lines [id:da6831470219253408] 
\draw    (511.5,16) -- (513,164) ;
%Straight Lines [id:da9172400887087635] 
\draw    (117.5,14) -- (511.5,16) ;
%Straight Lines [id:da24829736125231583] 
\draw    (117.5,14) -- (117.5,80) ;
\draw [shift={(117.5,82)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da304016495194801] 
\draw    (289.5,17) -- (290.46,65) ;
\draw [shift={(290.5,67)}, rotate = 268.85] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7211463196741601] 
\draw    (585,206) -- (649.5,205.03) ;
\draw [shift={(651.5,205)}, rotate = 539.14] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (119,114) node [anchor=north west][inner sep=0.75pt]   [align=left] {NN1};
% Text Node
\draw (271.46,105) node [anchor=north west][inner sep=0.75pt]   [align=left] {NN2};
% Text Node
\draw (47,100) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \theta _{I}$};
% Text Node
\draw (194,126) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \theta _{U}$};
% Text Node
\draw (327.46,188) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{46.378108000000005pt}\setlength\topsep{0pt}
\begin{center}
Barrier 
\end{center}
certificate
\end{minipage}};
% Text Node
\draw (370,88) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle a$};
% Text Node
\draw (274,208) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle x$};
% Text Node
\draw (511,186) node [anchor=north west][inner sep=0.75pt]   [align=left] {\begin{minipage}[lt]{29.930608000000003pt}\setlength\topsep{0pt}
\begin{center}
SMT\\solver
\end{center}

\end{minipage}};
% Text Node
\draw (120,25) node [anchor=north west][inner sep=0.75pt]   [align=left] {retrain with $\displaystyle \theta _{I}$};
% Text Node
\draw (294.5,25) node [anchor=north west][inner sep=0.75pt]   [align=left] {retrain with $\displaystyle \theta _{I} ,\theta _{U}$};
% Text Node
\draw (583,178) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle certificate$};
% Text Node
\draw (415,181) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle certificate$};


\end{tikzpicture}

